Controllable Shape Modeling with Neural Generalized Cylinder

Neural shape representation, such as neural signed distance field (NSDF), becomes more and more popular in shape modeling as its ability to deal with complex topology and arbitrary resolution. Due to the implicit manner to use features for shape representation, manipulating the shapes faces inherent challenge of inconvenience, since the feature cannot be intuitively edited. In this work, we propose neural generalized cylinder (NGC) for explicit manipulation of NSDF, which is an extension of traditional generalized cylinder (GC). Specifically, we define a central curve first and assign neural features along the curve to represent the profiles. Then NSDF is defined on the relative coordinates of a specialized GC with oval-shaped profiles. By using the relative coordinates, NSDF can be explicitly controlled via manipulation of the GC. To this end, we apply NGC to many non-rigid deformation tasks like complex curved deformation, local scaling and twisting for shapes. The comparison on shape deformation with other methods proves the effectiveness and efficiency of NGC. Furthermore, NGC could utilize the neural feature for shape blending by a simple neural feature interpolation.

==> Figures/4_discussion_radius_blend.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.7\linewidth]{Figures/image/4_discussion_radius_blend.png}
    \caption{The effect of radius blending.}
    \label{fig:4_discussion_radius_blend}
\end{figure}

==> Figures/4_exp_reprpower.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/image/4_exp_reprpower.png}
    \caption{Representation Power. }
    \label{fig:4_exp_reprpower}
\end{figure*}

==> Sections/6_extra_figs.tex <==
\newpage
% \input{Figures/4_exp_reprpower}
\input{Figures/4_exp_transform_curve}
\input{Figures/4_exp_scale_tilt}
\input{Figures/4_exp_mix_part}
\input{Figures/4_exp_deform_comparison}
\input{Figures/4_exp_generation}


==> Tables/4_exp_time_cost.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{lccccc}
    \hline
         & Dolphin & CAD & Spoon & Bar1 & Bar2 \\
    \hline
    |V| & 27950 & 5255 & 12394 & 14872 & 14872 \\
    \hline
    ARAP & 1.46s & 0.32s & 0.713s & 0.807s & 0.763s \\
    NFGP & 7584s & 7484s & 8650s & 7697s & 7706s \\
    Ours & 1.172s & 2.148s & 1.576s & 1.105s & 1.063s \\
    \hline
    \end{tabular}
    \caption{Time cost, |V|: number of vertices.}
    \label{tab:time_cost}
\end{table}
